Pig aggression classification using CNN, Transformers and Recurrent Networks

The development of techniques that can be used to analyze and detect animal behavior is a crucial activity for the livestock sector, as it is possible to monitor the stress and animal welfare and contributes to decision making in the farm. Thus, the development of applications can assist breeders in making decisions to improve production performance and reduce costs, once the animal behavior is analyzed by humans and this can lead to susceptible errors and time consumption. Aggressiveness in pigs is an example of behavior that is studied to reduce its impact through animal classification and identification. However, this process is laborious and susceptible to errors, which can be reduced through automation by visually classifying videos captured in controlled environment. The captured videos can be used for training and, as a result, for classification through computer vision and artificial intelligence, employing neural network techniques. The main techniques utilized in this study are variants of transformers: STAM, TimeSformer, and ViViT, as well as techniques using convolutions, such as ResNet3D2, Resnet(2+1)D, and CnnLstm. These techniques were employed for pig video classification with the objective of identifying aggressive and non-aggressive behaviors. In this work, various techniques were compared to analyze the contribution of using transformers, in addition to the effectiveness of the convolution technique in video classification. The performance was evaluated using accuracy, precision, and recall. The TimerSformer technique showed the best results in video classification, with median accuracy of 0.729.

==> ajustes.tex <==
\newcommand{\nomeEditor}{Spyros Fountas}
\newcommand{\nomeArtigo}{Pig aggression classification using CNN, Transformers and Recurrent Networks}
\newcommand{\nomeRevista}{Smart Agricultural Technology}
\newcommand{\nomeAutor}{Junior Silva Souza}


==> textos/introducao.tex <==



Com o aumento da demanda mundial por proteína, a criação de suínos vem sendo ampliada com o financiamento de cooperativas que buscam produzir em larga escala para suprir o mercado. Entretanto, em modelos tradicionais de criação voltados à alta produtividade, o comportamento dos animais pode ser afetado por fatores de estresse, o que pode acabar reduzindo a produtividade. Assim sendo, é necessário o acompanhamento técnico do comportamento animal, para garantir que os fatores de estresse presentes no ambiente de criação não levem à comportamentos prejudiciais à produtividade. Portanto, soluções técnicas que priorizem o acompanhamento do comportamento animal são cada vez mais utilizadas ~\cite{shao2021pig}.

O comportamento animal é um fator que deve ser analisado por todos os criadores de suínos em suas granjas durante o ciclo de produção. A investigação, a análise e o acompanhamento dos animais permitem encontrar informações úteis à melhoria do bem-estar animal e, consequentemente, ao aumento da produção~\cite{alameer2020automatic}.

A agressividade, alimentação e  monta são alguns dos comportamentos mais observados pelos criadores de suínos de corte e requerem atenção e observação técnica. Assim, acompanhar os animais em diversos momentos, procurando encontrar alterações na postura é uma rotina desempenhada por criadores. Em geral, trata-se de uma atividade manual, realizada visualmente, e que necessita de experiência e conhecimentos técnicos. Além disso, trata-se de uma atividade altamente suscetível a erros~\cite{alameer2020automatic}.


Nos últimos anos, a observação do comportamento animal vem sendo automatizada por meio de técnicas de Visão Computacional (VC) e Inteligência Artificial (IA). Essas técnicas podem ser utilizadas para classificar, localizar e rastrear, por exemplo, animais em grupo~\cite{xu2022automatic}. Nas criações, sua implementação se dá com o uso de câmeras para capturar imagens (fotos) ou vídeos, ou ambos, e enviá-las para uma central, onde é realizado o processamento, pelo qual podem ser identificadas eventuais anomalias~\cite{ma2022basic}.

Por meio de vídeos, é possível capturar informações acerca de eventos que ocorrem ao longo de um determinado período e que podem indicar  comportamentos característicos, desejáveis ou indesejáveis, para a criação de suínos. A agressividade é um dos  comportamentos indesejáveis, não pode ser identificada facilmente a partir de uma única imagem. Nesse caso, a análise de vídeos pode trazer melhores resultados, por incidir também sobre informações temporais. A ideia fundamental  deste trabalho é que o comportamento agressivo pode ser identificado por meio de informações espaciais (extraídas de um quadro) e temporais (extraídas de sequências de quadros).


Neste trabalho, serão avaliadas técnicas de classificação de vídeos. Mais especificamente, serão avaliadas as seguintes versões de modelos baseados em \textit{transformer} para processamento de vídeos: \textit{Visual Vision Transformer} (\textit{ViViT}), \textit{Space Time Attention Model} (\textit{STAM}) e \textit{TimeSformer}. Além disso, também foi analisada uma rede de convolução com recorrência. Tendo em vista a identificação do comportamento animal agressivo. A performance dos algoritmos elencados foi analisada com base em quatro métricas usuais de classificação: acurácia, precisão, revocação e medida-f.

Neste trabalho, serão avaliadas técnicas de classificação de vídeos. Mais especificamente, serão avaliadas as seguintes versões de modelos baseados em \textit{transformer} para processamento de vídeos: \textit{Visual Vision Transformer} (\textit{ViViT}), \textit{Space Time Attention Model} (\textit{STAM}) e \textit{TimeSformer}. Além disso, também foi testada uma rede convolucional com recorrência. Tendo em vista a identificação do comportamento animal agressivo, a performance dos algoritmos foi analisada com base em quatro métricas usuais de classificação: acurácia, precisão, revocação e medida-f.

==> textos/materialMetodo.tex <==



% References in https://languagetool.org/pt-BR
Para a realização deste trabalho, foi construída uma base de vídeos coletados em uma propriedade particular no estado de Mato Grosso do Sul, Brasil, com animais em regime de engorda com aproximadamente 80 dias. As imagens foram coletadas durante o primeiro semestre de 2022, a uma temperatura média de 28\textcelsius. Os períodos de captura dos vídeos se concentraram nos primeiros horários da manhã, em torno das 8h00 às 10h00, e nos últimos horários da tarde, em torno das 13h00 às 16h00, foram períodos em que os animais estão em maior atividade.


\subsection{Banco de Vídeos}

O banco tem 353 vídeos, dos quais 84 foram anotados como ``agressivo'' e 269 foram anotados como ``não agressivo''. Os vídeos foram coletados a uma altura de aproximadamente 2,60 metros e a uma distância de 5 metros de cada baia em relação à câmera em diagonal. O dispositivo de câmera utilizado foi um Motorola e(6i) configurado para ter quadros com altura de 2340 píxeis e largura de 4160 píxeis, no espaço de cor RGB e com uma taxa de 30 quadros por segundo e períodos de 30 minutos.

Os vídeos dos animais foram analisados e recortados, representando duas classes de eventos: agressivo e não agressivo. Em média, cada video contém 80 quadros. Os vídeos foram classificados manualmente no formato utilizado nos conjuntos de dados kinetics \footnote{Formato descrito em \url{https://www.deepmind.com/open-source/kinetics}.}. Assim, os vídeos foram salvos em uma pasta, juntamente com um arquivo que descreve o nome do vídeo, quantidade de quadros e a classe correspondente. Nas Figuras \ref{fig:agressivo} e \ref{fig:naoagressivo}, podemos visualizar duas amostras de vídeos classificados como agressivo e não agressivo, respectivamente. Durante a gravação,  a luz do sol iluminava o galpão lateralmente e,  como parte da lateral é fechada por uma lona azul, as imagens apresentavam uma tonalidade azulada.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=250px, height=50px]{img/agressivo.jpg}
    \caption{Uma amostra de um vídeo contendo 8 quadros que apresentam um suíno tentando morder a calda de outro animal.}
    \label{fig:agressivo}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=250px, height=50px]{img/nao-agressivo.jpg}
    \caption{Uma amostra de um vídeo contendo 8 quadros que apresentam animais em comportamento não agressivo.}
    \label{fig:naoagressivo}
\end{figure}

\subsection{Pré-processamento dos vídeos}

A compressão de vídeo foi utilizada para reduzir a quantidade de quadros a serem processados, removendo as informações redundantes. Em \citet{liu2020computer}, a redução de quadros foi analisada e executada para encontrar a quantidade mínima e suficiente de quadros necessários para o treinamento e  classificação. Esse processo permite uma redução do processamento durante o treinamento e evita informações redundantes, já que a variação no posicionamento e a velocidade dos animais entre um quadro e outro pode ser mínima.


A redução de quadros foi efetuada a uma taxa de 3x1, ou seja, cada sequência de 30 quadros foi reduzida para 10 quadros. Uma representação esquemática da redução pode ser vista na figura~\ref{fig:compress}. Com uma redução de 3x1, um vídeo de 80 quadros é convertido em um vídeo de 26 quadros. Além disso, cada quadro do vídeo foi redimensionado para ter 400 pixeis de altura e 400 pixeis de largura.


 \begin{figure}[!htp]
     \centering
     \includegraphics[scale=0.5,width=\linewidth]{img/representacao_compressao_video.pdf}
     \caption{Representação da compressão de um vídeo na taxa 3x1. Cada vídeo de entrada com 80 quadros foi reduzido para 26 quadros.}
     \label{fig:compress}
 \end{figure}


\subsection{Redes Profundas}

Nesse trabalho foi realizada a comparação da performance de redes neurais profundas aplicadas à classificação de vídeos, contemplando técnicas com convolução e redes de recorrência bem como técnicas que utilizam \textit{transformers}. As redes neurais convolucionais (CNN) foram utilizadas em conjunto com redes neurais recorrentes  e são uma alternativa  na classificação de vídeos, em trabalhos como~\cite{cnnlstmOnly} e \cite{patil2021video} foi proposto o desenvolvimento de classificadores de vídeos utilizando  redes convolucionais e recorrência.  A CNN  utilizada para a extração de atributos em cada quadro do vídeos, representando a informação espacial e a rede utilizada foi a \textit{resnet}. Enquanto que a rede recorrência (LSTM) foi utilizada para realizar a classificação em si a partir da informações extraídas de cada quadro, representando a informação temporal. 


Os \textit{transformers}, por outro lado, são implementações de mecanismos de atenção desenvolvidos e utilizados inicialmente no campo do processamento de linguagem natural, e posteriormente foram adaptados para  visão computacional em classificação, detecção e segmentação de imagens e vídeos \cite{9574462Bi}. 

No processamento de linguagem natural, cada palavra é descrita na forma de \textit{tokens}. Já em visão computacional, uma imagem é dividida em pequenas partes (denominadas patches), a partir das quais são gerados os\textit{tokens}. O uso de \textit{transformers} em visão computacional teve inicio após a introdução do ViT (\textit{Vision Transformers}) na classificação de imagens.

O ViT propõe a construção de uma rede neural que usa \textit{transformer}, sendo uma adaptação pura prescindindo de convoluções~\cite{dosovitskiy2020image, vitOnly}. Nele, os tokens são extraídos de uma imagem e passam pelo \textit{transformer encoder}, um dos dois blocos que formam o \textit{transformer} original. Um dos diferenciais do \textit{transformer} é seu mecanismo de atenção, o \textit{dot product attention}, presente no \textit{encoder}. Os \textit{encoders} são responsáveis por extrair informações, e um \textit{Multilayer Perceptron} (\textit{MLP}) é responsável pela classificação.    


A arquitetura ViViT (\textit{Video Vision Transformers})
é uma aplicação de ViT em problemas de classificação de vídeos e imagens. Nessa arquitetura, cada vídeo é considerado uma sequência de imagens das quais podem ser extraídas informações espaciais e temporais importantes para a classificação. Como um  vídeo é composto por imagens sequenciais (quadros), a cada mudança de quadro as imagens sofrem alterações que podem ser utilizadas para obter informações relevantes. Além disso, cada quadro em um vídeo analisado por ViT também contribui com um conjunto de informações espaciais que podem ser compartilhadas entre todas as imagens e utilizada para a extração da informação temporal. A arquitetura ViViT possui dois níveis de aplicação de ViT o primeiro nível é  aplicado em  cada imagem em um vídeo. O segundo nível é aplicado aos resultados obtidos do nível anterior \cite{Arnab_2021_ICCV}.

A arquitetura STAM (\textit{Space Time Attention Model}) é semelhante à arquitetura ViViT, uma vez que aplica o ViT para extrair informações espaciais e temporais separadamente. Isso aumenta a eficiência  de processamento, ao mesmo tempo que  prioriza a extração da informação espacial antes da informação temporal. Na arquitetura STAM são selecionados 16 quadros por vídeo \cite{stamOnly} para o processamento.


A arquitetura TimeSformer (\textit{Time-Space Transformer}) divide cada frame de um vídeo em patches de tamanho de 16x16, podendo variar entre 32x32, 64x64, entre outros tamanhos. Essa arquitetura  utiliza ViT  para extrair informações espaciais e temporais  dos patches obtidos. Durante o processamento, apenas os patches mais informativos são selecionados. A quantidade e a localização dos patches pode variar durante o processamento que passa para a execução múltiplos ViT. Esse processo permite que o modelo se concentre nas partes mais importantes de cada frames para realizar a classificação de vídeo \cite{timeSformerOnly}.


\subsection{Delineamento experimental}


As quatro arquiteturas foram testadas por meio de validação cruzada em 10 dobras \cite{liu2019margin}. A cada dobra, 10\% das imagens pertencentes ao conjunto de treinamento foram utilizadas para validação. Os quadros dos vídeos foram redimensionados para $(128, 128)$ pixels. Para os módulos de \textit{transformer}, foram extraídos 32 patches de cada quadro. Cada arquitetura foi testada com  as seguintes taxas de aprendizagem: 0,001 e 0,0003 valores escolhidos e utilizados em trabalhos como \cite{islam2020human} e \cite{s19173738} que aplicaram em diferentes tipos de otimizadores. O otimizador  utilizado foi o Adam (\textit{Adaptative momentum}), \cite{desai2020comparative} e \cite{almadani} utilizaram nos experimentos e obtiveram melhores resultados.

O treinamento foi realizado em 20 épocas com \textit{batch size} definido em 10 conforme \cite{10042233Zhou}. Ao final do treinamento de cada rede em cada dobra as redes foram testadas e foram obtido valores para as quatro métricas de performance acurácia, precisão, revocação e medida-f.


No nosso experimento os pesos da redes foram inicializados aleatoriamente. O treinamento foi realizado ao longo de 20 épocas, com um \textit{batch size} definido em 10, conforme descrito em \cite{10042233Zhou}. Ao final do treinamento de cada rede em cada dobra, as redes foram testadas, e foram obtidos valores para as quatro métricas de desempenho: acurácia, precisão, revocação e medida-F.

==> textos/resultados.tex <==

As Tabelas ~\ref{tab:accuracy}, ~\ref{tab:precision}, ~\ref{tab:recall} e ~\ref{tab:fmeasure} mostram, respectivamente os valores de acurácia, precisão, revocação e medida-f referentes às técnicas de classificação de vídeo utilizadas.Os resultados apresentados levam em consideração a taxa de aprendizado de 0.0001, com os valores médios obtidos no experimento com validação cruzada em 10 folds. As colunas representam o nome da técnica, os valores de média, mediana e desvio padrão (SD). A técnica CNNLSTM  apresentou  os melhores resultados em relação a todas as métricas utilizadas.

The ANOVA results were highly significant for the techniques in all four metrics, with $p$-values of approximately $0$. The Scott-Knott clustering test indicated that CNN-LSTM is better than the others in all metrics. In precision, it achieved the highest mean, despite being clustered together with ViViT. ViViT achieved the worst performance in all metrics, except in precision, which had STAM figure in the last place. For learning rates, only the recall result was significant ($p=0.02097$), in which case the Scott-Knott test indicated that $0.0003$ leads to a better performance. The ANOVA results were not significant for the interaction between architectures and learning rates in any metric.


\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \toprule
        \multicolumn{4}{|c|}{Accuracy} \\ \hline
        {Technique} &     Mean &   Median &       SD \\
        \midrule
        cnnlstm    &    \textbf{0.887} &    \textbf{0.891} &    0.046 \\
        stam       &    0.720 &    0.722 &    \textbf{0.086} \\
        timesforme &    0.667 &    0.675 &    0.085 \\
        vivit      &    0.662 &    0.672 &    0.074 \\
        \bottomrule
    \end{tabular}
    \caption{The results are presented for all techniques using the accuracy metric.}
\label{tab:accuracy}
\end{table}

O melhor resultado em termos de acurácia foi obtido pela técnica CNNLSTM, como pode ser visto na Tabela ~\ref{tab:accuracy}, com um valor médio de 0.887 e um desvio padrão baixo em comparação com as outras técnicas, assim como ocorre em todas as outras métricas. Em contrapartida, a técnica STAM apresentou o segundo maior resultado em termos de mediana e média, porém com um desvio padrão maior em comparação aos outros valores.

\begin{table}[!htp]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \toprule
    \multicolumn{4}{|c|}{Precision} \\ \hline
    {Technique} &      Mean &    Median &        SD \\
    \midrule
        cnnlstm    &     \textbf{0.903} &     \textbf{0.903} &     0.046 \\
        stam       &     0.778 &     0.766 &     0.110 \\
        timesforme &     0.830 &     0.863 &     \textbf{0.195} \\
        vivit      &     0.888 &     0.926 &     0.113 \\
    \bottomrule
    \end{tabular}
    \caption{The results are presented for all techniques using the precision metric.}
    \label{tab:precision}
\end{table}

A técnica vivit apresentou o segundo melhor resultado em relação à métrica de precisão, com um valor médio de 0.903, como pode ser observado na Tabela ~\ref{tab:precision}. Isso demonstra um bom desempenho na classificação de verdadeiros positivos nos vídeos. Já em relação ao recall e à medida-f, a técnica STAM apresentou os melhores resultados, como indicado em suas respectivas tabelas.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \toprule
    \multicolumn{4}{|c|}{Recall} \\ \hline
    Technique &   Mean &     Median &       SD \\
    \midrule
    cnnlstm    &  \textbf{0.868} &  \textbf{0.873} &  0.055 \\
    stam       &  0.637 &  0.656 &  0.161 \\
    timesforme &  0.423 &  0.476 &  \textbf{0.195} \\
    vivit      &  0.389 &  0.406 &  0.167 \\
    \bottomrule
    \end{tabular}
    \caption{The results are presented for all techniques using the recall metric.}
    \label{tab:recall}
\end{table}


Analisando a Tabela ~\ref{tab:fmeasure}, podemos observar que a técnica CNNLSTM apresentou o menor desvio padrão em todos os testes, o que indica regularidade nos resultados. Por outro lado, a técnica STAM apresentou o segundo maior desvio padrão, indicando variação entre os resultados.


\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \toprule
    \multicolumn{4}{|c|}{F-Measure} \\ \hline
    Technique &   Mean &     Median &       SD \\
    \midrule
    cnnlstm    & \textbf{0.885} & \textbf{0.883} & 0.047 \\
    stam       &          0.686 &          0.690 & 0.116 \\
    timesforme &          0.531 &          0.582 & \textbf{0.198} \\
    vivit      &          0.513 &          0.553 &  0.178 \\
    \bottomrule
    \end{tabular}
    \caption{The results are presented for all techniques using the F-Measure metric.}
    \label{tab:fmeasure}
\end{table}


Uma matriz de confusão foi gerada a partir do conjunto de dados teste com a técnica CNNLSTM, como podemos visualizar na Figura~\ref{fig:cnnlstm}. Os resultados demonstram uma maior acertividade com os vídeos que compreende a classe não agressivo.


\begin{figure}[!ht]
    \centering
    \includegraphics[scale=0.4]{img/cnnlstm.png}
    \caption{Resultado da Matriz de confusão obtida no conjunto de teste com a técnica CNNLSTM.}
    \label{fig:cnnlstm}
\end{figure}


==> textos/trabalhoCorrelato.tex <==


Pesquisas sobre a aplicação de redes neurais artificiais a tarefas de visão computacional permitiram o desenvolvimento de novas tecnologias de extração, classificação, segmentação e detecção de objetos em imagens com alta performance. A aplicação dessas novas tecnologias ao comportamento animal tem sido tema de trabalhos diversos. Em alguns casos, as aplicações têm dialogado com áreas que vão além da visão computacional. Em ~\citet{liao2022domestic}, por exemplo, foi proposto o reconhecimento do comportamento de suínos através da conversão de sons em imagens, utilizando \textit{transformers} e redes de convolução. 

%Aplicações que envolvem contagem de animais são exemplos como em \cite{huang2021center} que realizou a detecção de leitões em imagens, utilizando segmentação semântica. 


Em \citet{jast} foi desenvolvida a detecção do comportamento associado à hidratação e a alimentação. Os autores utilizaram a rede de detecção YOLOv3 (\textit{You Only Look Once}) e suas variantes para a detecção do comportamento dos animais. Utilizando CNN (\textit{Convolution Neural Network}) \citet{hansen2021towards} realizaram um trabalho de classificação de humor de suínos através de imagens faciais. \citet{shigang2021pig} também realizou a detecção e classificação de leitões através de imagens da face. 


As imagens são a base das redes de classificação, permitindo que um conjunto de dados sejam extraídos e analisados pela rede para detectar características úteis na classificação. Entretanto, o comportamento animal requer uma visualização mais profunda das imagens, assim, a utilização de vídeos é uma opção é mais interessante. Em \citet{ZHANG2019104884} foi utilizada a rede de detecção SSD (\textit{Single-Shot Detector}) para detectar o comportamento a partir vídeos, os autores avaliariam a viabilidade de uma mudança na arquitetura para realizar a detecção de objetos. Já os autores \citet{zhang2020automated}  utilizaram a convolução em vídeos para realizar a classificação do comportamento animal em 5 categorias: dormindo, monta, deitado, comendo e andando. A proposta trouxe a utilização de fluxo óptico que é uma técnica que utiliza informação a partir do movimento utilizado em paralelo as redes de convolução aplicáveis tanto em vídeos no espaço de cor RGB quanto utilizando o fluxo óptico. 

A detecção e o acompanhamento de animais também foi analisado por \cite{fernandez2020computer} que realizou a identificação e o acompanhamento de animais através de CNN e filtro de kalman, os autores propuseram um mecanismo para monitorar o movimento de suínos para analisar o deslocamento dos animais. 

O comportamento animal associado a agressividade deve ser acompanhado e estudado para permitir o bem-estar animal e como consequência garantir maior produção. Os animais podem apresentar o comportamento relacionado, por exemplo, a agressividade por uma série de fatores que podem estar associado a alimentação, estresse, espaço, etc. Cabe ao criador realizar o monitoramento e o acompanhamento dos animais para evitar perdas \cite{yang2020review}. As técnicas clássicas de CNN para classificação e a detecção de vídeos não conseguem extrair em simultâneo, informações temporais e espaciais, obtidas em um determinado tempo. Tais informações, como a agressividade, que ocorre em um curto espaço de tempo e requer a extração de informações relacionadas entre as imagens que compõe o vídeo, são importantes na classificação.

Em \citet{wang2021pca} foi utilizada uma rede CNN com LSTM (\textit{Long Short-Term Memory}) buscando extrair informação espacial e temporal para realizar a classificação da postura de porcas com leitões em baias. Os autores utilizaram PCA para reduzir a quantidade de quadros e realizar o treinamento da rede. Enquanto \cite{chen2020computer} propuseram a construção de uma rede de convolução com recorrência para  analisar a interação de suínos com diferentes objetos distribuídos no local. A inserção de objetos para que os animais possam interagir permitiu a redução do estresse e aumentou o bem-estar animal.

Um diferencial na classificação de vídeos foi abordado por \cite{hu2021dual}, através da utilização e a aplicação do conceito de atenção para realizar a segmentação de imagens e que depois foi ampliado para a classificação. O uso de atenção na classificação de imagem permitiu o desenvolvimento de técnicas que implementam mecanismos que destacam pontos importantes do vídeo e a relação entre eles \cite{vaswani2017attention} e \cite{dai2021dynamic}. Assim com o conceito de atenção em imagens surgiram as primeiras aplicações de tranformers em visão computacional. Em \citet{dosovitskiy2020image} foi proposto aplicar o conceito em imagens e expandido para vídeos \cite{multViT}.

A classificação de vídeos é uma atividade que requer a extração de informação temporal e espacial. Essa informação pode ser extraída por técnicas como redes de convolução e recorrência. Nesse trabalho foi proposto o uso da técnicas de \textit{transformers}  e convolução com recorrência para analisar o desempenho.
